An Approach for Handling Missing Attribute Values in Attribute-Based Access Control Policy Mining

Attribute-Based Access Control (ABAC) enables highly expressive and flexible access decisions by considering a wide range of contextual attributes. ABAC policies use logical expressions that combine these attributes, allowing for precise and context-aware control. Algorithms that mine ABAC policies from legacy access control systems can significantly reduce the costs associated with migrating to ABAC. However, a major challenge in this process is handling incomplete entity information, where some attribute values are missing. This paper introduces an approach that enhances the policy mining process by predicting or inferring missing attribute values. This is accomplished by employing a contextual clustering technique that groups entities according to their known attributes, which are then used to analyze and refine authorization decisions. By effectively managing incomplete data, our approach provides security administrators with a valuable tool to improve their attribute data and ensure a smoother, more efficient transition to ABAC.

==> evolutionary-alg.tex <==
% !TeX root = main.tex

\section{Evolutionary Algorithm}
\label{sec:evol-alg}

\newcommand{\mergeandsimplifyEvol}{{\rm mergeRulesAndSimplify2}}

Our evolutionary algorithm is based on the evolutionary algorithm for ReBAC mining (without incompleteness or noise) in \cite{bui19mining}, which is inspired by Medvet et al.'s work \cite{medvet2015}.  It is in the context-free grammar genetic programming (CFGGP) paradigm\fullonly{ \cite{gramEvolSurvey2010}}, in which individuals, which in our context are ReBAC rules, are represented as derivation trees of a context-free grammar (CFG).  The main part of the algorithm is preceded by {\it grammar generation}, which specializes the generic grammar of \ourlang to a specific input, so that rules in the language of the grammar contain only classes, fields, constants, and actions that appear in the input, and all path expressions are type-correct and satisfy the same length limits as in the greedy algorithm.

The algorithm's first phase iterates over the given entitlements, and uses each of the selected entitlements as the seed for an evolutionary search that adds one new rule to the candidate policy.  Each evolutionary search starts with an initial population containing candidate rules created from a seed tuple in a similar way as in the greedy algorithm along with numerous random variants of those rules together with some completely random candidate rules, evolves the population by repeatedly applying genetic operators (mutations and crossover), and then selects the highest quality rule in the population as the result of that evolutionary search.  The second phase improves the candidate rules by further mutating them.

% To save space, we omit some unchanged details.

\begin{figure}[tbp]
\begin{tabular}[t]{@{}l@{}}
// \com{Phase 1: Construct candidate policy, using evolutionary search to create each rule.}\\
$\Rules = \emptyset$; $\uncovsp = \spa_0.\Copy()$\\
\whileloop\ $\uncovsp$ is not empty\\
\ind $\seed$ = highest-quality entitlement in $\uncovsp$\shortonly{ (same quality metric as in greedy algorithm)}\fullonly{ using $\QspL$ metric}\\
\ind {\it pop} = initialPopulation($\seed, \Rules, \uncovsp$)\\
\ind \forloop\ ${\it gen}$ = 1 to {\it nGenerationsSearch}\\
\ind\ind $\op$ = a genetic operator randomly selected from {\it searchOps}\\
% the following selection uses a uniform distribution
\ind\ind $S$ = set of {\it nTournament} rules randomly selected from {\it pop}\\
\ind\ind \ifstmt\ $op$ is a mutation\\
% type mutation can create a not-well-formed rule.  in this case, we abort the mutation.
% to avoid mentioning this explicitly, we can model this by saying that the effect of
% applying $op$ in this case is to return the original rule.
\ind\ind\ind {\it pop}.add(the rule generated by applying $op$ to the highest-quality rule in $S$)\\
\ind\ind\elsestmt\ ~~~ // \com{$op$ is a cross-over}\\
\ind\ind\ind {\it pop}.add(the two rules generated by applying $op$ to the two highest-quality rules in $S$)\\
\ind\ind\eifstmt\\
\ind\ind remove the lowest-quality rules in {\it pop} until $\vert {\it pop}\vert$ = {\it popSize}\\
\ind \eforloop\\
\ind $\rho$ = the highest-quality rule in {\it pop}\\
\ind \ifstmt\ $\alphavalid(\rho)$;\\
\ind\ind \Rules.add($\rho$); \uncovsp.removeAll($\mean{\rho}$)\\
\ind \eifstmt\\
\ewhileloop\\
// \com{Phase 2: Improve the candidate rules by further mutating them.}\\
\foreachloop\ $\rho$ \forloopin\ \Rules\\
\ind\forloop\ ${\it gen}$ = 1 to {\it nGenerationsImprove}\\
%\ind\ind // \com{If no improvements are found in the first {\it nGenerationsImprove}/2 attempts, give up.}\\
\ind\ind \ifstmt\ {\it gen} = {\it nGenerationsImprove}/2 $\land$ (all attempted improvements to $\rho$ failed)\\
\ind\ind\ind \breakstmt\ \ // \com{This rule is unlikely to improve.  Don't bother trying more.}\\
\ind\ind\eifstmt\\
\ind\ind $\op$ = a genetic operator randomly selected from {\it improveOps}\\
\ind\ind $\rho'$ = the rule generated by applying $op$ to $\rho$\\
% for consistency with the treatment of not-well-formed rules in phase 1, we will assume that the check of whether \rho' is well-formed is done as part of applying $op$, and that the original rule is returned if the mutated rule is not well-formed
\ind\ind \ifstmt\ $\alphavalid(\rho') \,\land\, \IDL(\rho')\le\IDL(\rho)$\\
\ind\ind\ind ${\it redundant} = \setc{\rho_0\in\Rules}{\mean{\rho_0}\subseteq\mean{\rho'}}$\\
\ind\ind\ind\ifstmt\ $(\Rules\union\set{\rho'}\setminus {\it redundant})$ covers $\spa_0$ and has lower WSC than $\Rules$\\
\ind\ind\ind\ind \Rules.removeAll({\it redundant}); \Rules.add($\rho'$)\\
\ind\ind\ind\eifstmt\\
\ind\ind\eifstmt\\	
\ind\eforloop\\
\eforloop\\
%Note: we use rule quality metric from ReBAC Miner for mergeAndSimplify
\fullonly{\mergeandsimplifyEvol(\Rules)}\shortonly{Repeatedly call $\mergerulesL(\Rules)$ and $\simplifyrulesL(\Rules)$ until they have no further effect}\\
\return\ the rules in \Rules\ with quality at least $\tau$
\end{tabular}
\caption{Evolutionary algorithm for extended ReBAC policy mining problem. 
Inputs: subject-permission relation $\spa_0$, class model $\cm$, object model $\om$.  Output: set of rules $\Rules$.\fullonly{  The algorithm also has numerical parameters that determine population size, number of generations, etc., as described in the text.}}
\label{fig:evol-alg}\vspace{-1.5ex}
\end{figure}

Pseudocode appears in Figure \ref{fig:evol-alg}.  Function initialPopulation($\tuple{s,r,a}, \Rules, \uncovsp$) creates an initial population for the evolutionary search for a high-quality rule that covers the seed $\tuple{s,r,a}$ and other tuples.  It is implicitly parameterized by the desired population size {\it popSize}. Half of the initial population is generated as follows: perform the same two calls to $\addcandidateruleL$ as in Figure \ref{fig:greedy}, add those rules to the initial population, and then add random variants of those rules obtained by removing some atomic conditions and atomic constraints.  The other half consists of rules with subject type $\type(s)$ or one of its ancestors (selected randomly), resource type $\type(r)$ or one of its ancestors, randomly generated conditions and constraint, and action set $\set{a}$. 

Rule quality is measured using a fitness function $f$, modified from the one in \cite{bui19mining} to take missing assignments into account using a threshold approach: false acceptances are ignored unless they exceed a threshold specified by algorithm parameter $\alpha$.  The fitness function is $f(\rho, \alpha) = \tuple{\far(\rho,\alpha),\frr(\rho),\IDL(\rho),\wsc(\rho)}$.  The {\em false acceptance rate} $\far(\rho,\alpha)$
is 0 if $\frac{|\mean{\rho}\setminus\spa_0|}{|\mean{\rho}|} < \alpha$ and is 
$\frac{|\mean{\rho}\setminus\spa_0|}{|\mean{\rho}|}$ otherwise.
The {\em false rejection rate} is $\frr(\rho)=|\uncovsp\setminus\mean{\rho}|$, and $\hypertarget{ID}{\ID(\rho)}$ is the number of atomic conditions in $\rho$ with path ``id''.\fullonly{  The fitness ordering is lexicographic order on these tuples, where smaller is better.}

The two validity checks used in the algorithm in \cite{bui19mining} are replaced with $\alphavalidity$ checks, as shown in Figure \ref{fig:evol-alg}.  Also, to deal with excess entitlements, the algorithm returns only rules with quality at least $\tau$.

The set {\it searchOps} of genetic operators used in the search phase contains the two traditional CFGGP genetic operators: a mutation operator that randomly selects a non-terminal in the derivation tree being evolved, and replaces the existing subtree rooted at that non-terminal with a new subtree randomly generated starting from that non-terminal, and a cross-over operator that randomly selects a non-terminal that appears in both of the derivation trees being evolved (called ``parents''), and swaps the subtrees rooted at that non-terminal.  It also contains a {\em double mutation} operator that mutates two out of the three predicates (the subject condition, resource condition, and constraint) in a rule (this enables the operator to have an effect similar to \generalizeruleL), and a {\em simplify mutation} that removes one randomly selected atomic condition or atomic constraint (this mutation is included to increase the overall probability of these mutations).
The set {\it improveOps} of genetic operators used in the improvement phase is similar, except it also contains a {\it type mutation} operator that can replace the subject type or resource type with one of its ancestors.

\fullonly{We describe the genetic operators as if they directly manipulate abstract syntax trees, because this allows a higher-level and more intuitive presentation.  However, the genetic operators actually manipulate derivation trees of the generated grammar.}

% searchOpDist: 0.1 for crossover, approx 0.24 each for single, action, and simplify mutation, approx 0.17 for double mutation.  these sum to 0.99.

\shortonly{The version of $\simplifyrulesL$ used in this algorithm is the same as in the greedy algorithm except extended with an additional simplification: replace the subject type or resource type with one of its children, if the policy still covers $\spa_0$.}\fullonly{Function $\mergeandsimplifyEvol$ is the same as $\mergeandsimplifyL$ except that it incorporates one additional simplification: replace the subject type or resource type with a child of that type, if the policy still covers $\spa_0$.}

% the need for this simplification (i.e., a rule whose type is ``too general'') did not arise in experiments with greedy alg, so we did not bother to introduce it there.
% similarly, we don't call mergeRulesInheritance in evolutionary alg because the need for it (i.e., candidate policy containing two rules with sibling types that need to be merged into one rule with parent type) did not arise in experiments with evolutionary alg.

